Scheduling to Learn In An Unsupervised Online Streaming Model

An unsupervised online streaming model is considered where samples arrive in an online fashion over $T$ slots. There are $M$ classifiers, whose confusion matrices are unknown a priori. In each slot, at most one sample can be labeled by any classifier. The accuracy of a sample is a function of the set of labels obtained for it from various classifiers. The utility of a sample is a scalar multiple of its accuracy minus the response time (difference of the departure slot and the arrival slot), where the departure slot is also decided by the algorithm. Since each classifier can label at most one sample per slot, there is a tradeoff between obtaining a larger set of labels for a particular sample to improve its accuracy, and its response time. The problem of maximizing the sum of the utilities of all samples is considered, where learning the confusion matrices, sample-classifier matching assignment, and sample departure slot decisions depend on each other. The proposed algorithm first learns the confusion matrices, and then uses a greedy algorithm for sample-classifier matching. A sample departs once its incremental utility turns non-positive. We show that the competitive ratio of the proposed algorithm is $\frac{1}{2}-{\mathcal O}\left(\frac{\log T}{T}\right)$.

==> Scheduling to learn in unsupervised online streaming model/DetailedSimulations.tex <==
\subsection{Detailed Experiments}
%\vspace{-.15in}
In this section, we provide the empirical study comparing the competitive ratio and the regret between Algorithm \ref{alg:greedy-genie} and \ref{alg:realgreedy}. Ideally, we would like to include the optimal algorithm as well, however, since it is unknown, we have to preclude that. 
We perform three sets of experiments, first on synthetic dataset, and next two on real datasets, 
the binary Bird dataset \cite{bird} which has labels of bird species, and the multi-class DOG dataset \cite{dog} which has labels for the dog breeds. 

For all the experiments, the utility with Algorithm \ref{alg:greedy-genie} is computed assuming the true values of confusion matrices are available at the first slot, while for Algorithm \ref{alg:realgreedy}, the first $T_L$ slots are used for learning the confusions matrices, the utility is computed over the remaining $T-T_L$ slots using the learnt confusion matrices.


%to capture the regret of Algorithm \ref{alg:realgreedy} against Algorithm \ref{alg:greedy-genie}, we plot the utility over all the $T$ slots for Algorithm \ref{alg:greedy-genie}, assuming true values of confusion matrices are available at the first slot, while for Algorithm \ref{alg:realgreedy}, the first $T_L$ slots are used for learning the confusions matrices, and 
% in terms of total utility, of 
%the \textit{Algorithm 1} and \textit{Algorithm 2} mentioned in section 3 above. In all the respective experiments followed
%we cap the respective total running time to some $T$ and evaluate the performance of \textit{Algorithm 1} and \textit{Algorithm 2},
%where \textit{Algorithm 1} runs for the entire time horizon $T$ since it's given the confusion matrices and \textit{Algorithm 2} 
%first learns the confusion matrices for some time and then follows the \textit{Greedy} algorithm. The evaluations are made on
%one synthetic dataset and two real datasets.
%\vspace{-0.1in}
%\subsection{
%\vspace{-0.1in}
{\bf Synthetic Data:} We consider $M= 30$ classifiers/workers, and samples arrive over the time horizon $T$. We consider that each 
sample can belong to either of two classes $\{1,2\}$, and the true label of each sample is $\{1,2\}$ with equal probability. 
The number of incoming samples in a slot follows a Poisson distribution with rate $5$, and the sample weights $w_{s}$ are 
chosen uniformly randomly from the set $[3,4,\dots, 10]$.
For each classifier, the $2\times2$ confusion matrix is generated as follows: the diagonal entries $\bP_m(i,i)$ is given by $p_{m}= 0.9- 0.005 \times m$, $m=1,\dots, 30$, and the off-diagonal entries of $\bP_m$ are obtained as $1-p_m$. 
%The obtained $30$ confusion matrices are then shuffled randomly and assigned to $30$ classifiers.


In Fig. \ref{fig:synth}, for a fixed time horizon $T=10000$, we plot the accuracy ($\infty-norm$ of the error) in learning the confusion matrices with learning intervals of length $T_L \in \{5, 15, 25, 45, \cdots 1250\}$ using procedure Online Learn. We also plot the resulting utilities of Algorithm \ref{alg:greedy-genie} (that knows $p_m$ ahead of time) and Algorithm \ref{alg:realgreedy} (that works with learnt values of $p_m$ after $T_L$ slots),  in Fig. \ref{fig:synth}. Note that even though no learning is used for Algorithm \ref{alg:greedy-genie}, the utility curve is not constant because of inherent randomness in number of arriving samples in each slot, and their weights $w_s$.
%
%From Fig. \ref{fig:synth}, we can clearly see that as the length of the learning interval $T_L$ increases, the utility of Algorithm \ref{alg:realgreedy} 
% initially increases on account of better accuracy of confusion matrices, however, when $T_L$ is sufficiently 
%large, the utility starts to decrease since a  lot of time slots are wasted in learning the confusion matrices during which Algorithm \ref{alg:realgreedy} accrues no utility compared to Algorithm \ref{alg:greedy-genie}. 

In Fig. \ref{fig:synthregret}, we plot the regret (normalized with the average number of samples arriving per time slot, and average weight of any sample to identify the scaling with $T$) and the competitive ratio between Algorithm \ref{alg:greedy-genie} and Algorithm \ref{alg:realgreedy}, as a function of time horizon $T$, where for each value of $T$, the best learning interval $T_L$ is found. Fig. \ref{fig:synthregret} shows that the simulated performance is better than the theoretical results; regret is $o(\log T)$ and the competitive ratio is at least $1/2-\log(T)/T$.

%\vspace{-.3in}

%Algorithm Thus, choosing $T_L$ appropriately, one can infer from Fig. \ref{fig:synth}, that the regret of Algorithm \ref{alg:realgreedy} over Algorithm \ref{alg:greedy-genie} is lower than 
%($\sim (\log T)$) promised by Corollary \ref{cor:expregret}.

%\\\\
%After the data is generated the experiment is performed as follows, a. we fix the total time horizon $T$ as 10,000, b.1 Incoming data is sent to \textit{Algorithm 1} and \textit{Algorithm 2}, b.2 \textit{Algorithm 1} keeps generating utility throughout the time horizon, while \textit{Algorithm 2} trades initial utility by using initial incoming samples to learn its confusion matrices till $n_{i}$ time units,
%c.1 now for first set of data we have $n_{1}= 5$ or we send samples across 5 time units to all the workers for labelling, c.2 the labels obtained are passed through the \textit{Opt-D&S} algorithm mentioned in \cite{4} to learn the confusion matrices for \textit{Algorithm 2}, d. from time $n_{1}$ onward both \textit{Algorithm 1} and \textit{Algorithm 2} generate utility, e. we keep on doing this process for all binary tasks with
%$n \in \{5, 15, 25, 35, 45, 50, 150, 250, 350, 450, 500, 750, 1000, 1250\}$.
%\\\\
%We perform 5 iterations, for each binary task with reserved $n_{i}$ time slots, of the above mentioned process to get better estimate of the utility from both \textit{Algorithm 1} and \textit{Algorithm 2}. The main evaluation is with regards to the total utility generated, across all the incoming samples, by passing the samples via \textit{Algorithm 1} and \textit{Algorithm 2}. Even before running the simulations common logic would suggest that for algorithm 2 there's a trade-off between time spent learning and gain in utility. Which is exactly what we see in out simulation results.

\begin{figure}[h]
\centering
\includegraphics[width= .65\linewidth]{normalized_syn_data_regret_ratio.png}
\caption{Regret and competitive ratio for Algorithm \ref{alg:realgreedy} and Algorithm \ref{alg:greedy-genie} with  synthetic data}
\label{fig:synthregret}
\end{figure}
\begin{figure}
\centering
\includegraphics[width= 0.8\linewidth]{paper_synthetic2.png}
\caption{Total Utility and Infinity norm as a function of learning time for synthetic data}
\label{fig:synth}
\end{figure}

%\begin{minipage}{.5\textwidth} %

%\end{minipage}
%\subsection{}
%For real data experiments, we compare the algorithms on two datasets: the binary Bird dataset \cite{5} which has labels of bird species, and the multi-class DOG dataset \cite{6} which has labels for the breed of a dog.
{\bf Real Data Sets:}Next, we use real two datasets, the Bird dataset \cite{bird} that has $M= 39$ classifiers/workers, and $|S|=108$ samples in total, and the DOG dataset \cite{dog} for which 
we take $M= 90$ classifiers and $|S|=798$ samples in total. 
We modified the multi-class DOG dataset to a binary dataset by clubbing classes 
$1,2$ as class $1$ and classes $3,4$ as class $2$. 
Similar to Fig. \ref{fig:synth}, we first plot the utilities of  Algorithm \ref{alg:greedy-genie} and Algorithm  \ref{alg:realgreedy} for a fixed value of time horizon $T=4000$, together with the accuracy of learnt confusion matrices in Figs. \ref{fig:bird} and Fig. \ref{fig:dog}, for the Bird and the DOG datasets, respectively.
To simulate genie access of $p_m$ for Algorithm \ref{alg:greedy-genie}, the confusion matrix 
learnt after using all the samples is taken as the input at the start itself. 
In Figs. \ref{fig:birdregret} and  \ref{fig:dogregret}, we plot the regret (normalized) and the competitive ratio between Algorithm \ref{alg:greedy-genie} and Algorithm \ref{alg:realgreedy}, as a function of time horizon $T$, where for each value of $T$, the best learning interval $T_L$ is found. More detailed results can be found in the Appendix.
%Figs. \ref{fig:birdregret} and \ref{fig:dogregret} again show that the simulated performance is better than the theoretical results.

%For both these datasets, we plot the regret  and the competitive ratio between Algorithm \ref{alg:greedy-genie} and Algorithm \ref{alg:realgreedy}, as a function of time horizon $T$
%use time horizon of $T=4000$, while all other details are as described above. 
%
%As a function of $T_L$, we plot the utilities of Algorithm \ref{alg:greedy-genie} and \ref{alg:realgreedy} in Fig. \ref{fig:bird} and Fig. \ref{fig:dog}, for the two data sets, and infer the same conclusion about the regret as in the case of synthetic data set.
% 
%Our experimental results on real datasets are consistent with the results from synthetic datasets. There is indeed a trade-off between time spent learning and total utility. One peculiar thing to observe from the results of DOG dataset \cite{6} however is that in its case the confusion matrices are very well learnt since the beginning due to high number of samples, 252, which are required due to sparsity of the dataset and due to the fact that we require each worker to label at least one sample. 


\begin{figure}
%\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{paper_bluebird2.png}
  \caption{Utility and accuracy with BIRD data set v/s $T_L$.}
  \label{fig:bird}
\end{figure}%

\begin{figure}[!h]
\centering
\includegraphics[width= 0.65\linewidth]{normalized_bluebird_data_regret_ratio.png}
\caption{Regret and competitive ratio for Algorithm \ref{alg:realgreedy} and Algorithm \ref{alg:greedy-genie} with  Bird data set }
\label{fig:birdregret}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=.9\linewidth]{paper_DOG1.png}
  \caption{Utility and accuracy with DOG data set v/s $T_L$.}
  \label{fig:dog}
\end{figure}
%\vspace{-.1in}
\begin{figure}[!h]
\centering
\includegraphics[height= 0.4\linewidth]{normalized_dog_data_regret_ratio.png}
\caption{Regret and competitive ratio for Algorithm \ref{alg:realgreedy} and Algorithm \ref{alg:greedy-genie} with  DOG data set }
\label{fig:dogregret}
\end{figure}


==> Scheduling to learn in unsupervised online streaming model/input.tex <==
%\usepackage{fancyhdr}
%\pagestyle{fancy}

\usepackage{amsfonts}
\usepackage{times}
%\usepackage[pdftex]{graphicx}
%\DeclareGraphicsExtensions{.jpg}
%\usepackage[dvips]{graphicx}
%\DeclareGraphicsExtensions{.eps}
\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{amsmath}
%\usepackage{cite}
\usepackage{verbatim}
\newtheorem{theorem}{Theorem}
%
\newtheorem{acknowledgement}[theorem]{Acknowledgement}
%\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{axiom}[theorem]{Axiom}
\newtheorem{case}[theorem]{Case}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{criterion}[theorem]{Criterion}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{summary}[theorem]{Summary}
\newtheorem{remark}[theorem]{Remark}
\newenvironment{proof}{ \textbf{Proof:} }{ \hfill $\Box$}

\newcommand{\figref}[1]{{Fig.}~\ref{#1}}
\newcommand{\tabref}[1]{{Table}~\ref{#1}}
\newcommand{\bookemph}[1]{ {\em #1}}
\newcommand{\Ns}{N_s}
\newcommand{\Ut}{U_t}
\newcommand{\fig}[1]{Fig.\ \ref{#1}}
\def\onehalf{\frac{1}{2}}
\def\etal{et.\/ al.\/}
\newcommand{\bydef}{\triangleq}
\newcommand{\tr}{{\it{tr}}}
\def\SNR{{\textsf{SNR}}}

% blackboard lowercase
\def\bydef{:=}
\def\bba{{\mathbb{a}}}
\def\bbb{{\mathbb{b}}}
\def\bbc{{\mathbb{c}}}
\def\bbd{{\mathbb{d}}}
\def\bbee{{\mathbb{e}}}
\def\bbff{{\mathbb{f}}}
\def\bbg{{\mathbb{g}}}
\def\bbh{{\mathbb{h}}}
\def\bbi{{\mathbb{i}}}
\def\bbj{{\mathbb{j}}}
\def\bbk{{\mathbb{k}}}
\def\bbl{{\mathbb{l}}}
\def\bbm{{\mathbb{m}}}
\def\bbn{{\mathbb{n}}}
\def\bbo{{\mathbb{o}}}
\def\bbp{{\mathbb{p}}}
\def\bbq{{\mathbb{q}}}
\def\bbr{{\mathbb{r}}}
\def\bbs{{\mathbb{s}}}
\def\bbt{{\mathbb{t}}}
\def\bbu{{\mathbb{u}}}
\def\bbv{{\mathbb{v}}}
\def\bbw{{\mathbb{w}}}
\def\bbx{{\mathbb{x}}}
\def\bby{{\mathbb{y}}}
\def\bbz{{\mathbb{z}}}
\def\bb0{{\mathbb{0}}}



\def\opt{\mathsf{OPT}}
\def\on{\mathsf{ON}}
\def\off{\mathsf{OFF}}
% Bold lowercase
\def\bydef{:=}
\def\ba{{\mathbf{a}}}
\def\bb{{\mathbf{b}}}
\def\bc{{\mathbf{c}}}
\def\bd{{\mathbf{d}}}
\def\bee{{\mathbf{e}}}
\def\bff{{\mathbf{f}}}
\def\bg{{\mathbf{g}}}
\def\bh{{\mathbf{h}}}
\def\bi{{\mathbf{i}}}
\def\bj{{\mathbf{j}}}
\def\bk{{\mathbf{k}}}
\def\bl{{\mathbf{l}}}
\def\bm{{\mathbf{m}}}
\def\bn{{\mathbf{n}}}
\def\bo{{\mathbf{o}}}
\def\bp{{\mathbf{p}}}
\def\bq{{\mathbf{q}}}
\def\br{{\mathbf{r}}}
\def\bs{{\mathbf{s}}}
\def\bt{{\mathbf{t}}}
\def\bu{{\mathbf{u}}}
\def\bv{{\mathbf{v}}}
\def\bw{{\mathbf{w}}}
\def\bx{{\mathbf{x}}}
\def\by{{\mathbf{y}}}
\def\bz{{\mathbf{z}}}
\def\b0{{\mathbf{0}}}

% Bold capital letters
\def\bA{{\mathbf{A}}}
\def\bB{{\mathbf{B}}}
\def\bC{{\mathbf{C}}}
\def\bD{{\mathbf{D}}}
\def\bE{{\mathbf{E}}}
\def\bF{{\mathbf{F}}}
\def\bG{{\mathbf{G}}}
\def\bH{{\mathbf{H}}}
\def\bI{{\mathbf{I}}}
\def\bJ{{\mathbf{J}}}
\def\bK{{\mathbf{K}}}
\def\bL{{\mathbf{L}}}
\def\bM{{\mathbf{M}}}
\def\bN{{\mathbf{N}}}
\def\bO{{\mathbf{O}}}
\def\bP{{\mathbf{P}}}
\def\bQ{{\mathbf{Q}}}
\def\bR{{\mathbf{R}}}
\def\bS{{\mathbf{S}}}
\def\bT{{\mathbf{T}}}
\def\bU{{\mathbf{U}}}
\def\bV{{\mathbf{V}}}
\def\bW{{\mathbf{W}}}
\def\bX{{\mathbf{X}}}
\def\bY{{\mathbf{Y}}}
\def\bZ{{\mathbf{Z}}}
\def\b1{{\mathbf{1}}}


% Blackboard capital letters
\def\bbA{{\mathbb{A}}}
\def\bbB{{\mathbb{B}}}
\def\bbC{{\mathbb{C}}}
\def\bbD{{\mathbb{D}}}
\def\bbE{{\mathbb{E}}}
\def\bbF{{\mathbb{F}}}
\def\bbG{{\mathbb{G}}}
\def\bbH{{\mathbb{H}}}
\def\bbI{{\mathbb{I}}}
\def\bbJ{{\mathbb{J}}}
\def\bbK{{\mathbb{K}}}
\def\bbL{{\mathbb{L}}}
\def\bbM{{\mathbb{M}}}
\def\bbN{{\mathbb{N}}}
\def\bbO{{\mathbb{O}}}
\def\bbP{{\mathbb{P}}}
\def\bbQ{{\mathbb{Q}}}
\def\bbR{{\mathbb{R}}}
\def\bbS{{\mathbb{S}}}
\def\bbT{{\mathbb{T}}}
\def\bbU{{\mathbb{U}}}
\def\bbV{{\mathbb{V}}}
\def\bbW{{\mathbb{W}}}
\def\bbX{{\mathbb{X}}}
\def\bbY{{\mathbb{Y}}}
\def\bbZ{{\mathbb{Z}}}

% Caligraphic capital letters
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

% Sans serif capital letters
\def\sfA{\mathsf{A}}
\def\sfB{\mathsf{B}}
\def\sfC{\mathsf{C}}
\def\sfD{\mathsf{D}}
\def\sfE{\mathsf{E}}
\def\sfF{\mathsf{F}}
\def\sfG{\mathsf{G}}
\def\sfH{\mathsf{H}}
\def\sfI{\mathsf{I}}
\def\sfJ{\mathsf{J}}
\def\sfK{\mathsf{K}}
\def\sfL{\mathsf{L}}
\def\sfM{\mathsf{M}}
\def\sfN{\mathsf{N}}
\def\sfO{\mathsf{O}}
\def\sfP{\mathsf{P}}
\def\sfQ{\mathsf{Q}}
\def\sfR{\mathsf{R}}
\def\sfS{\mathsf{S}}
\def\sfT{\mathsf{T}}
\def\sfU{\mathsf{U}}
\def\sfV{\mathsf{V}}
\def\sfW{\mathsf{W}}
\def\sfX{\mathsf{X}}
\def\sfY{\mathsf{Y}}
\def\sfZ{\mathsf{Z}}


% sans serif lowercase
\def\bydef{:=}
\def\sfa{{\mathsf{a}}}
\def\sfb{{\mathsf{b}}}
\def\sfc{{\mathsf{c}}}
\def\sfd{{\mathsf{d}}}
\def\sfee{{\mathsf{e}}}
\def\sfff{{\mathsf{f}}}
\def\sfg{{\mathsf{g}}}
\def\sfh{{\mathsf{h}}}
\def\sfi{{\mathsf{i}}}
\def\sfj{{\mathsf{j}}}
\def\sfk{{\mathsf{k}}}
\def\sfl{{\mathsf{l}}}
\def\sfm{{\mathsf{m}}}
\def\sfn{{\mathsf{n}}}
\def\sfo{{\mathsf{o}}}
\def\sfp{{\mathsf{p}}}
\def\sfq{{\mathsf{q}}}
\def\sfr{{\mathsf{r}}}
\def\sfs{{\mathsf{s}}}
\def\sft{{\mathsf{t}}}
\def\sfu{{\mathsf{u}}}
\def\sfv{{\mathsf{v}}}
\def\sfw{{\mathsf{w}}}
\def\sfx{{\mathsf{x}}}
\def\sfy{{\mathsf{y}}}
\def\sfz{{\mathsf{z}}}
\def\sf0{{\mathsf{0}}}

\def\Nt{{N_t}}
\def\Nr{{N_r}}
\def\Ne{{N_e}}
\def\Ns{{N_s}}
\def\Es{{E_s}}
\def\No{{N_o}}
\def\sinc{\mathrm{sinc}}
\def\dmin{d^2_{\mathrm{min}}}
\def\vec{\mathrm{vec}~}
\def\kron{\otimes}
\def\Pe{{P_e}}
\newcommand{\expeq}{\stackrel{.}{=}}
\newcommand{\expg}{\stackrel{.}{\ge}}
\newcommand{\expl}{\stackrel{.}{\le}}
\def\SIR{{\mathsf{SIR}}}

% Added by Takao
\def\nn{\nonumber}





==> Scheduling to learn in unsupervised online streaming model/intro.tex <==
\section{Introduction}
Dawid and Skene in what is now regarded as seminal work \cite{dawid1979maximum}, considered the basic problem of discovering ground truth or true labels of samples from multiple but possibly erroneous/noisy responses/measurements. The more modern paradigm considers the online variant of Dawid and Skene's model
for unsupervised learning (USL), where samples arrive over time and the problem is to discover their true labels using a large number of classifiers, typically
 `non-expert' crowdsourcing workers. 
With the advancement in cloud based services, this model has been successfully implemented in 
variety of platforms, such as Amazon Mechanical Turk.

Such systems, however, have limitations resulting from  the lack of knowledge of ground truth and the precise accuracy information of each of the classifiers. 
Thus, there is a need for aggregating algorithms that can infer the ground truth using a large ensemble of classifiers. There is a large 
body of work in this direction, where the main idea is to find a small set of good classifiers and/or estimating the accuracy of all classifiers from the obtained labels for different samples \cite{li2013error, raykar2010learning, shaham2016deep, karger2011iterative, ho2012online, 
natarajan2013learning, jordan, whitehill2009whose, liu2015online, gong2018incentivizing, nordio2018selecting, karger2014budget, 
sheng2008get}. 

To make the model formal, a confusion matrix $\bP$ is defined for each classifier, whose $i,j^{th}$ entry captures the probability that 
the classifier labels a sample as belonging to class $j$ when the true class label is $i$. Learning the confusion matrix for each classifier is part of the problem, using which the true label of a sample can be discovered with high probability. 

In this paper, we consider a competition model for the online USL in the Dawid-Skene model, where in each time slot, a set of samples arrive into the system. There are a total of 
$M$ classifiers, where  classifier $m$ is defined by its true confusion matrix $\bP_m$, that is unknown a priori. 
Without loss of generality, we consider that each classifier can label at most one sample in each time slot. See Remark \ref{rem:cap} for more details. The accuracy of a sample in a time slot  is defined as the probability of classifying it correctly using the optimal combining rule given its label set obtained till that time slot. 
 To consider a general model, we let that a sample can remain in system for more than one time slot to increase its accuracy in hope of getting more labels, however, at the cost of accruing delay. 
% Thus, the utility of each sample is the 
%
%
%To 
%Each sample ideally wants to get labeled by as many `good' classifiers as possible, however, Thus, there is a competition between samples for getting labeled by multiple classifiers as quickly as possible.
% 
Thus, this model captures the tradeoff between sample accuracy and throughput of the system, where throughput is defined as the rate of sample departures.

The studied model is well-suited for real-time learning paradigms, such as image classification in social networks e.g. instagram, facebook, automated crowd controlling system, medical diagnostics, automated quality management in factories, large dataset handling applications in bioinformatics, etc., where not only good classification is needed but the speed/delay incurred matters. In the interest of space, we refer the reader to \cite{massoulie2016capacity, shah2020adaptive} for more discussion on applications.

\subsection{Related Work}
For USL models, the competition between accuracy and throughput has been studied in prior work \cite{massoulie2016capacity, shah2020adaptive, shakkott} by defining a metric called {\it capacity}. Capacity is defined to be the largest stochastic rate 
of arrival of samples per time slot, such that each sample can be guaranteed to have an accuracy above a certain threshold with high probability, 
while maintaining queue stability. 
Queue stability states that the long term average of the expected number of samples in the system (yet to depart the system) remains bounded. 
%A more refined question was addressed more recently in \cite{shakkott}, where the capacity region was defined as the set of all (arrival rate, accuracy) tuples, 
%such that the system is stable for the chosen arrival rate and a given lower bound on the accuracy of each sample with high probability. The quest in \cite{shakkott} is to find the Pareto frontier of the capacity region. 
Even though the prior work \cite{massoulie2016capacity, shah2020adaptive,shakkott} captures the 
tension between accuracy of samples and their arrival rates, it only considers the metric of stability that is a long term throughput metric, and cannot account for more refined utilities such as per sample delay, etc. 


To model a more fine grained system, in this work, we define a  per-sample utility, that is a function of the accuracy of that sample, 
and the time it takes to accrue that accuracy. Accuracy is directly related to the set of classifiers that label that sample. Thus, 
each sample would ideally like to get labels from the set of good or all classifiers, however, that requires waiting for multiple time slots because of the presence of other samples and each classifier labelling at most one sample per unit time, introducing a delay cost. In particular, we choose the sample utility to be a linear combination of its accuracy at its departure time, and the response time (departure time -arrival time), and the total utility is the sum of the utilities of all samples. 


Thus, in each time slot, the problem is to find a matching between the outstanding samples and the classifiers, 
given the current estimates on the entries of the confusion matrices of each classifier, such that the overall utility is maximized. Even when the confusion matrices are perfectly known a priori, this problem is combinatorial and hard to solve. The problem becomes even more involved in the practical setting, since the quality of estimates of the confusion matrices depend on the prior matching decisions, while future matching decisions depend on the current estimates of the confusion matrices. 

To formulate the problem in the online setting, we use the metric of {\it competitive ratio} that is defined as the ratio of the utility of any algorithm and the utility of the optimal offline algorithm, minimized over all input sequences of samples. The optimal offline algorithm is assumed to have genie knowledge (perfect knowledge of the confusion matrices) and knows the entire input sequence non-causally. Thus, in contrast to \cite{massoulie2016capacity, shah2020adaptive,shakkott},  in this paper, we consider that the sample arrival sequence is arbitrary and not necessarily stochastic (e.g. Poisson).


\subsection{Our contributions}
\begin{itemize}[leftmargin=*]
\item With genie knowledge of the confusion matrices, we define a greedy algorithm and show that its competitive ratio is at least $\frac{1}{2}$. The main tool in deriving this result is to show that the utility of each sample is submodular, for which the greedy algorithm's competitive ratio is shown to be at least $\frac{1}{2}$ using results from recent work  \cite{nived} compared to classical work \cite{fisher1978analysis}. 

\item Next, we define a {\bf regret} metric between the greedy algorithm with genie knowledge and the greedy algorithm that has to learn the confusion matrices. We show that if the error between the estimate and the true value of the entries of the confusion matrices is small enough, then the matching decisions made by the greedy algorithm in the genie setting and the greedy algorithm after learning are identical. This allows us to show that the expected regret of the greedy algorithm that learns the confusion matrices is at most ${\mathcal O}(\log(T))$, where $T$ is the time horizon.
 
 \item Combining the above two results, we get our final result that the competitive ratio of the proposed greedy algorithm that also learns the confusion matrices is at least $\frac{1}{2}-{\mathcal O}\left(\frac{\log T}{T}\right)$.
 \item We also provide experimental results for both the synthetic and the real-world data sets to confirm our theoretical results.
 
\end{itemize}

==> Scheduling to learn in unsupervised online streaming model/simulationsedited.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}
%
%\usepackage[margin=1.5in]{geometry}    % For margin alignment
%\usepackage[english]{babel}
%% \usepackage[utf8]{inputenc}
%% \usepackage{algorithm}
%\usepackage[ruled]{algorithm2e}
%
%% \usepackage{arevmath}     % For math symbols
%\usepackage[noend]{algpseudocode}
%
%
%% \documentclass{article}
%% \usepackage[utf8]{inputenc}
%\usepackage{amsmath}
%% \usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{lipsum}
%\usepackage{amsthm}
%% \documentclass{article}
%% \usepackage[utf8]{inputenc}
%\usepackage{graphicx}
%\usepackage{subcaption} 
%\usepackage{float}
%% \usepackage[ruled,vlined]{algorithm2e}
%
%\usepackage{amsmath,amsfonts,amssymb,amsthm,epsfig,epstopdf,titling,url,array}
%
%
%\theoremstyle{plain}
%\newtheorem{thm}{Theorem}[section]
%\newtheorem{lem}[thm]{Lemma}
%\newtheorem{prop}[thm]{Proposition}
%\newtheorem*{cor}{Corollary}
%
%\theoremstyle{definition}
%\newtheorem{defn}{Definition}[section]
%\newtheorem{conj}{Conjecture}[section]
%\newtheorem{exmp}{Example}[section]
%\newtheorem{problem}{Problem}
%
%\theoremstyle{remark}
%% \newtheorem*{rem}{Remark}
%\newtheorem{rem}{Remark}
%\newtheorem*{note}{Note}


%
%\title{Simulations: Scheduling to learn}
%% \author{santanusrathod4415 }
%\date{August 2020}
%
%\begin{document}
%
%\maketitle
\vspace{-0.2in}
\section{Experiments}
\vspace{-.15in}
In this section, we provide the empirical study comparing the competitive ratio and the regret between Algorithm \ref{alg:greedy-genie} and \ref{alg:realgreedy}. Ideally, we would like to include the optimal algorithm as well, however, since it is unknown, we have to preclude that. 
We perform three sets of experiments, first on synthetic dataset, and next two on real datasets, 
the binary Bird dataset \cite{bird} which has labels of bird species, and the multi-class DOG dataset \cite{dog} which has labels for the dog breeds. 

For all the experiments, the utility with Algorithm \ref{alg:greedy-genie} is computed assuming the true values of confusion matrices are available at the first slot, while for Algorithm \ref{alg:realgreedy}, the first $T_L$ slots are used for learning the confusions matrices, the utility is computed over the remaining $T-T_L$ slots using the learnt confusion matrices.


%to capture the regret of Algorithm \ref{alg:realgreedy} against Algorithm \ref{alg:greedy-genie}, we plot the utility over all the $T$ slots for Algorithm \ref{alg:greedy-genie}, assuming true values of confusion matrices are available at the first slot, while for Algorithm \ref{alg:realgreedy}, the first $T_L$ slots are used for learning the confusions matrices, and 
% in terms of total utility, of 
%the \textit{Algorithm 1} and \textit{Algorithm 2} mentioned in section 3 above. In all the respective experiments followed
%we cap the respective total running time to some $T$ and evaluate the performance of \textit{Algorithm 1} and \textit{Algorithm 2},
%where \textit{Algorithm 1} runs for the entire time horizon $T$ since it's given the confusion matrices and \textit{Algorithm 2} 
%first learns the confusion matrices for some time and then follows the \textit{Greedy} algorithm. The evaluations are made on
%one synthetic dataset and two real datasets.
%\vspace{-0.1in}
%\subsection{
%\vspace{-0.1in}
{\bf Synthetic Data:} We consider $M= 30$ classifiers/workers, and samples arrive over the time horizon $T$. We consider that each 
sample can belong to either of two classes $\{1,2\}$, and the true label of each sample is $\{1,2\}$ with equal probability. 
The number of incoming samples in a slot follows a Poisson distribution with rate $5$, and the sample weights $w_{s}$ are 
chosen uniformly randomly from the set $[3,4,\dots, 10]$.
For each classifier, the $2\times2$ confusion matrix is generated as follows: the diagonal entries $\bP_m(i,i)$ is given by $p_{m}= 0.9- 0.005 \times m$, $m=1,\dots, 30$, and the off-diagonal entries of $\bP_m$ are obtained as $1-p_m$. 
%The obtained $30$ confusion matrices are then shuffled randomly and assigned to $30$ classifiers.


%In Fig. \ref{fig:synth}, for a fixed time horizon $T=10000$, we plot the accuracy ($\infty-norm$ of the error) in learning the confusion matrices with learning intervals of length $T_L \in \{5, 15, 25, 45, \cdots 1250\}$ using procedure Online Learn. We also plot the resulting utilities of Algorithm \ref{alg:greedy-genie} (that knows $p_m$ ahead of time) and Algorithm \ref{alg:realgreedy} (that works with learnt values of $p_m$ after $T_L$ slots),  in Fig. \ref{fig:synth}. Note that even though no learning is used for Algorithm \ref{alg:greedy-genie}, the utility curve is not constant because of inherent randomness in number of arriving samples in each slot, and their weights $w_s$.
%
%From Fig. \ref{fig:synth}, we can clearly see that as the length of the learning interval $T_L$ increases, the utility of Algorithm \ref{alg:realgreedy} 
% initially increases on account of better accuracy of confusion matrices, however, when $T_L$ is sufficiently 
%large, the utility starts to decrease since a  lot of time slots are wasted in learning the confusion matrices during which Algorithm \ref{alg:realgreedy} accrues no utility compared to Algorithm \ref{alg:greedy-genie}. 

In Fig. \ref{fig:synthregret}, we plot the regret (normalized with the average number of samples arriving per time slot, and average weight of any sample to identify the scaling with $T$) and the competitive ratio between Algorithm \ref{alg:greedy-genie} and Algorithm \ref{alg:realgreedy}, as a function of time horizon $T$, where for each value of $T$, the best (numerically optimized) learning interval $T_L$ is found. Fig. \ref{fig:synthregret} shows that the simulated performance is better than the theoretical results; regret is $o(\log T)$ and the competitive ratio is at least $1/2-\log(T)/T$.
\begin{figure}
\centering
\includegraphics[width= .65\linewidth]{normalized_syn_data_regret_ratio.png}
\caption{Regret and competitive ratio for Algorithm \ref{alg:realgreedy} and Algorithm \ref{alg:greedy-genie} with  synthetic data}
\label{fig:synthregret}
\end{figure}
%\vspace{-.3in}

%Algorithm Thus, choosing $T_L$ appropriately, one can infer from Fig. \ref{fig:synth}, that the regret of Algorithm \ref{alg:realgreedy} over Algorithm \ref{alg:greedy-genie} is lower than 
%($\sim (\log T)$) promised by Corollary \ref{cor:expregret}.

%\\\\
%After the data is generated the experiment is performed as follows, a. we fix the total time horizon $T$ as 10,000, b.1 Incoming data is sent to \textit{Algorithm 1} and \textit{Algorithm 2}, b.2 \textit{Algorithm 1} keeps generating utility throughout the time horizon, while \textit{Algorithm 2} trades initial utility by using initial incoming samples to learn its confusion matrices till $n_{i}$ time units,
%c.1 now for first set of data we have $n_{1}= 5$ or we send samples across 5 time units to all the workers for labelling, c.2 the labels obtained are passed through the \textit{Opt-D&S} algorithm mentioned in \cite{4} to learn the confusion matrices for \textit{Algorithm 2}, d. from time $n_{1}$ onward both \textit{Algorithm 1} and \textit{Algorithm 2} generate utility, e. we keep on doing this process for all binary tasks with
%$n \in \{5, 15, 25, 35, 45, 50, 150, 250, 350, 450, 500, 750, 1000, 1250\}$.
%\\\\
%We perform 5 iterations, for each binary task with reserved $n_{i}$ time slots, of the above mentioned process to get better estimate of the utility from both \textit{Algorithm 1} and \textit{Algorithm 2}. The main evaluation is with regards to the total utility generated, across all the incoming samples, by passing the samples via \textit{Algorithm 1} and \textit{Algorithm 2}. Even before running the simulations common logic would suggest that for algorithm 2 there's a trade-off between time spent learning and gain in utility. Which is exactly what we see in out simulation results.

%\begin{figure}
%\centering
%\includegraphics[width= 0.8\linewidth]{paper_synthetic2.png}
%\caption{Total Utility and Infinity norm as a function of learning time for synthetic data}
%\label{fig:synth}
%\end{figure}

%\begin{minipage}{.5\textwidth} %

%\end{minipage}
%\subsection{}
%For real data experiments, we compare the algorithms on two datasets: the binary Bird dataset \cite{5} which has labels of bird species, and the multi-class DOG dataset \cite{6} which has labels for the breed of a dog.
{\bf Real Data Sets:} Next, we use real two datasets, the Bird dataset \cite{bird} that has $M= 39$ classifiers/workers, and $|S|=108$ samples in total, and the DOG dataset \cite{dog} for which 
we take $M= 90$ classifiers and $|S|=798$ samples in total. 
We modified the multi-class DOG dataset to a binary dataset by clubbing classes 
$1,2$ as class $1$ and classes $3,4$ as class $2$. 
%Similar to Fig. \ref{fig:synth}, we first plot the utilities of  Algorithm \ref{alg:greedy-genie} and Algorithm  \ref{alg:realgreedy} for a fixed value of time horizon $T=4000$, together with the accuracy of learnt confusion matrices in Figs. \ref{fig:bird} and Fig. \ref{fig:dog}, for the Bird and the DOG datasets, respectively.
%To simulate genie access of $p_m$ for Algorithm \ref{alg:greedy-genie}, the confusion matrix 
%learnt after using all the samples is taken as the input at the start itself. 
In Figs. \ref{fig:birdregret} and  \ref{fig:dogregret}, we plot the regret (normalized) and the competitive ratio between Algorithm \ref{alg:greedy-genie} and Algorithm \ref{alg:realgreedy}, as a function of time horizon $T$, where for each value of $T$, the best learning interval $T_L$ is found. More detailed results on best $T_L$ etc. can be found in the Appendix.
%Figs. \ref{fig:birdregret} and \ref{fig:dogregret} again show that the simulated performance is better than the theoretical results.

%For both these datasets, we plot the regret  and the competitive ratio between Algorithm \ref{alg:greedy-genie} and Algorithm \ref{alg:realgreedy}, as a function of time horizon $T$
%use time horizon of $T=4000$, while all other details are as described above. 
%
%As a function of $T_L$, we plot the utilities of Algorithm \ref{alg:greedy-genie} and \ref{alg:realgreedy} in Fig. \ref{fig:bird} and Fig. \ref{fig:dog}, for the two data sets, and infer the same conclusion about the regret as in the case of synthetic data set.
% 
%Our experimental results on real datasets are consistent with the results from synthetic datasets. There is indeed a trade-off between time spent learning and total utility. One peculiar thing to observe from the results of DOG dataset \cite{6} however is that in its case the confusion matrices are very well learnt since the beginning due to high number of samples, 252, which are required due to sparsity of the dataset and due to the fact that we require each worker to label at least one sample. 


%\begin{figure}
%%\begin{subfigure}{.5\textwidth}
%  \centering
%  \includegraphics[width=.8\linewidth]{paper_bluebird2.png}
%  \caption{Utility and accuracy with BIRD data set v/s $T_L$.}
%  \label{fig:bird}
%\end{figure}%

\begin{figure}[!h]
\centering
\includegraphics[width= 0.65\linewidth]{normalized_bluebird_data_regret_ratio.png}
\caption{Regret and competitive ratio for Algorithm \ref{alg:realgreedy} and Algorithm \ref{alg:greedy-genie} with  Bird data set }
\label{fig:birdregret}
\end{figure}

%\begin{figure}
%  \centering
%  \includegraphics[width=.9\linewidth]{paper_DOG1.png}
%  \caption{Utility and accuracy with DOG data set v/s $T_L$.}
%  \label{fig:dog}
%\end{figure}
%\vspace{-.1in}
\begin{figure}[!h]
\centering
\includegraphics[height= 0.4\linewidth]{normalized_dog_data_regret_ratio.png}
\caption{Regret and competitive ratio for Algorithm \ref{alg:realgreedy} and Algorithm \ref{alg:greedy-genie} with  DOG data set }
\label{fig:dogregret}
\end{figure}


%\bibliographystyle{unsrt}  
%\bibliography{references}  %%% Remove comment to use the external .bib file (using bibtex).
%%% and comment out the ``thebibliography'' section.


%%% Comment out this section when you \bibliography{references} is enabled.
%\begin{thebibliography}{1}
%
%\bibitem{1}
%Not Just Age but Age and Quality of Information by
%Nived Rajaraman, Rahul Vaze, Goonwanth Reddy.
%\url{https://arxiv.org/abs/1812.08617}
%
%\bibitem{2}
%Pareto Optimal Streaming Unsupervised Classification by 
%Soumya Basu, Steven Gutstein, Brent Lance, Sanjay Shakkottai.
%\url{http://proceedings.mlr.press/v97/basu19a/basu19a.pdf}
%
%\bibitem{3}
%An Online Learning Approach to Improving the Quality of
%Crowd-Sourcing by Yang Liu, Mingyan Liu.
%\url{https://ieeexplore.ieee.org/document/7892023}
%
%\bibitem{4}
%Spectral Methods meet EM: A Provably Optimal Algorithm
%for Crowdsourcing by
%Yuchen Zhang, Xi Chen, Dengyong Zhou, Michael I. Jordan
%\url{https://arxiv.org/pdf/1406.3824.pdf}
%
%\bibitem{5}
%P. Welinder, S. Branson, S. Belongie, and P. Perona. The multidimensional wisdom of crowds.
%In Advances in Neural Information Processing Systems, volume 10, pages 2424–2432, 2010.
%
%\bibitem{6}
%J. Deng, W. Dong, R. Socher, L.-J. Li, K. Li, and L. Fei-Fei. Imagenet: A large-scale hier-
%archical image database. In IEEE Conference on Computer Vision and Pattern Recognition,
%2009.

%\end{thebibliography}


%\end{document}

